Large-Scale MIDI-based Composer Classification

Music classification is a task to classify a music piece into labels such as genres or composers. We propose large-scale MIDI based composer classification systems using GiantMIDI-Piano, a transcription-based dataset. We propose to use piano rolls, onset rolls, and velocity rolls as input representations and use deep neural networks as classifiers. To our knowledge, we are the first to investigate the composer classification problem with up to 100 composers. By using convolutional recurrent neural networks as models, our MIDI based composer classification system achieves a 10-composer and a 100-composer classification accuracies of 0.648 and 0.385 (evaluated on 30-second clips) and 0.739 and 0.489 (evaluated on music pieces), respectively. Our MIDI based composer system outperforms several audio-based baseline classification systems, indicating the effectiveness of using compact MIDI representations for composer classification.

==> old.tex <==

The size of MIDI files are only 0.03\% of 16-bit stereo 32 kHz audio recordings of GiantMIDI-Piano, indicating MIDI files are compact representation of piano audio recordings.

Timbre is decided by the way the symbolic representations are interpreted, e.g., the choice of instrument, playing techniques, and recording environments. Both the symbolic representation and the timbre play an important role in the perception of classification labels such as genre or mood, and the system may be able to learn a classification task more effectively if they are given disentangled. 
For popular music, especially, the official original `score' is rarely published. 

none of them are labeled for prevail categories such as genre or tags

Piano rolls are regardless of piano conditions and recording environments. Therefore piano rolls are suitable representations for composer classification.

The advantage of onset roll is that onsets plays an important roll when human perceiving music. 

Considering the MIDI representations are much compact representation compared to log mel spectrograms. We show that MIDI files are effective representations for composer classification. Table 

\begin{table}[t]
\centering
\caption{Averaged classification accuracy of different systems for 10-composer and 100-composer classification}
\label{table:avg_results}
\begin{tabular}{*{6}{c}}
 \toprule
 & Audio & Fr & On & Fr+On & Fr+On+Vel \\
 \midrule
 10-class & 0.589 & 0.573 & 0.571 & 0.598 & 0.604 \\
 100-class & 0.341 & 0.303 & 0.281 & 0.317 & 0.324 \\
 \bottomrule
\end{tabular}
\end{table}
